TensoSDF: Roughness-aware Tensorial Representation for Robust Geometry and Material Reconstruction

Reconstructing objects with realistic materials from multi-view images is problematic, since it is highly ill-posed. Although the neural reconstruction approaches have exhibited impressive reconstruction ability, they are designed for objects with specific materials (e.g., diffuse or specular materials). To this end, we propose a novel framework for robust geometry and material reconstruction, where the geometry is expressed with the implicit signed distance field (SDF) encoded by a tensorial representation, namely TensoSDF. At the core of our method is the roughness-aware incorporation of the radiance and reflectance fields, which enables a robust reconstruction of objects with arbitrary reflective materials. Furthermore, the tensorial representation enhances geometry details in the reconstructed surface and reduces the training time. Finally, we estimate the materials using an explicit mesh for efficient intersection computation and an implicit SDF for accurate representation. Consequently, our method can achieve more robust geometry reconstruction, outperform the previous works in terms of relighting quality, and reduce 50% training times and 70% inference time.

==> paper_table.tex <==
\begin{table}[!t]
	\renewcommand{\arraystretch}{1.1}
	\caption{\label{tab:notations} Notations.}
\begin{small}
 % \left
  \begin{tabular}{|l|c|l|}\hline
  \multicolumn{2}{|c|}{Mathematical notation }\\
	\hline
		$\Omega$      			                                   &full spherical domain \\ 
		$\Omega^+$      			                                     &upper spherical domain \\ 
        $\Omega^-$      			                                     &lower spherical domain \\ 
        $\bomega_i \cdot \bomega_o$
                    &dot product \\
        $\left\vert \bomega_i \cdot \bomega_o \right \vert$
                    &absolute value of the dot product \\
        
	%	$\omega_i \cdot \omega_o$      			                       &dot product \\ 
	%	$|\omega_i\cdot \omega_o|$      		                     	&absolute value of the dot product \\ 
         $o()$ & the infinitesimal of higher order \\
	%	$\left\langle\omega_i, \omega_o \right\rangle$      	&dot product clamped to 0 \\ 
	%	$\chi^{+}(a)$                                                 &Heaviside function: 1 if a > 0 and 0 if a $\leq$ 0 \\
		\hline
		 \multicolumn{2}{|c|}{Physical quantities used in microfacet models}\\
				\hline
		$\omega_g = (0,0,1)$ & geometric normal \\
		$\omega_m $ & microfacet normal \\
		$\omega_i $ & incident direction \\
		$\omega_o $ & outgoing direction \\
		$\Lambda(\omega)  $ &the Smith Lambda function \\
		$D(\omega_m)$ &normal distribution function \\
		$D_{\omega_i}(\omega_m)$ &visible normals’ distribution \\
		$F(\omega_i,\omega_m)$ &Fresnel factor \\
	%	$\bs$ & a shading point \\
		
		%$G_1(\omega,\omega_m)$ &masking function \\
		%$G_1^{\mathrm{local}}(\omega,\omega_m)$ & masking (local)\\
		%$G_1^{\mathrm{dist}}(\omega)$& masking (distant)\\
		$\rho(\omega_i,\omega_o)$& multiple-bounce BSDF with the cosine term\\
%  &\added{并且入射方向向下，而非向上}\\
	%	$G_S^{(k)}(\omega_i,\omega_o,\omega_h)$ & shadowing-masking term\\
	%	$P^{(k<n)})$ & \question{how to name it?}\\
		

	%	$f_r$      					  &bidirectional scattering distribution function \\ 
		\hline
%  \multicolumn{2}{|c|}{Volume samples}\\
%\hline
      %$\vec x_v$                     & position \\ 
      %$\vec d_v$                     & direction of incoming light \\
      %$I_v$                          & intensity of node $v$ \\
			%$f_v$                          & frequency factor of node $v$ \\
			%$S_v$                          & surface area of node $v$ \\
			%$A_v$                          & area of the octree leaf cell\\
		%\hline
  %\multicolumn{2}{|c|}{Camera ray samples}\\
%\hline
      %$P_k$                          & sample point on camera ray \\
      %$d_k$                          & depth of sample point $P_k$ \\
		%\hline
		\end{tabular}

\end{small}
\end{table}

==> pseudocode.tex <==
% \newcommand{\mycommfont}[1]{\small\texttt{\textcolor[HTML]{4D8F33}{#1}}}
% \SetCommentSty{mycommfont}

% We show pseudo-code of segment term evaluation in Algorithm \ref{alg:SegmentTerm}, BRDF evaluation in Algorithm \ref{alg:eval} and sample in Algorithm \ref{alg:sample}.

% \newpage

% \begin{algorithm}
% \caption{SegmentTerm}
% \label{alg:SegmentTerm}
% \Class(\tcp*[h]{Initialize $\Lambda_o$}){$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     \Def{$m \gets 1$} \;
%     \Def{$N \gets 0$} \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf(\tcp*[h]{Downwards}){$\Lambda_k < 0$} {
%         $N \gets N+1$\;
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\Comment{cache the results when sampled rays are only downwards}
%         }(\tcp*[h]{Upwards}){
        
%             \eIf{$m = 0$}{
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }(\tcp*[h]{Initialize g}){
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }

%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{

%         \If(\tcp*[h]{Return results if cached}){$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }
%         \KwRet{ s }\;
    
%     }
% }

% \end{algorithm}


% \begin{algorithm}
% \caption{Eval}
% \label{alg:eval}
% \Fn{$\mathrm{eval}(\omega_i,\omega_o)$}{
% $\mathrm{SegmentTerm} \  s(\Lambda(\omega_o))$\Comment{ initializing }
% $f \gets 0$\Comment{result}
% $k \gets 0$ \Comment{bounce}
% $w \gets 1$\Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%     $s.\mathrm{addBounce}(\Lambda(\bd_{k}))$\;
%     $k \gets k + 1$\;
%     \If{$k >= rrDepth$}{
%         \If{$\mathrm{rand}()>q$}{
%         break;
%         }
%     $w \gets {w \over q}$\Comment{russian roulette}
%     }
%     $f \gets f + w \cdot v(\bd_{k},\omega_o)\cdot s.\mathrm{getS_k}() $\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
%     ($\bd_{k+1}$,$p_k$) $ \gets $ sample($ \bd_{k} $)\;
%     $w \gets {w \cdot v(\bd_{k},\bd_{k+1}) \over p_k}$\;
% }
%         \KwRet{ f }\;
% }
% \end{algorithm}

% \begin{algorithm}
% \caption{Sample}
% \label{alg:sample}
% \KwResult{weight $w$ and direction $\bd_k$}
% \BlankLine
% $p \gets 1$  \Comment{pdf}
% $k \gets 0$  \Comment{bounce}
% $w \gets 1$  \Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%    ($\bd_k$,$p_k$,$w_k$) $ \gets $ sample($ \bd_{k-1} $)\;
%    $w \gets w \cdot w_k$\;
%    $p \gets p \cdot p_k$\;
%     \If{$\bd_k.z > 0$}{
%     $G_1 \gets \frac{1}{|\Lambda(\bd_k)|}$\;
%         \eIf(\tcp*[h]{the ray continues the tracing with $G_1$ as the probablity}){$\mathrm{rand()}<G_1$}
%         {
%             $p \gets p \cdot G_1$\;
%             break;
%         }{
%             $p \gets p \cdot (1-G_1)$\;
%         }
%     }
% $k \gets k+1$\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
% }
%    $w \gets w \cdot S_k(\bd_0,...,\bd_k)$\;
%    $w \gets {w \over p}$\;
% \end{algorithm}

% \newcommand{\mybox}[3]{
% \begin{tcolorbox}[arc = 0pt, outer arc = 0pt,
%     colback = #1!10!white, colframe = #1!70!black,
%     boxsep = 0pt, left = 2pt, right = 2pt, top = 2pt, bottom = 2pt,
%     boxrule = 0pt, bottomrule = 1pt, toprule = 1pt,width=#2]
% #3
% \end{tcolorbox}
% }

% \newpage

% \begin{algorithm}[h]
% \caption{SegmentTerm}
% \label{alg:coloredST}
% \Class{$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     $N \gets 0$ \;
%     $m \gets 1$ \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf{$\Lambda_k < 0$} {
%       \mybox{green}{24mm}{
%        % \begin{mybox}[width=30mm]
%        $N \gets N+1$\;
%         % \end{mybox}
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\;
%         }
%         }{
        
%     \mybox{yellow}{33.5mm}{
%             \eIf{$m = 0$}
%             {
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }{
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }
% \mybox{red}{32mm}{
%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }}
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{
%     \mybox{cyan}{33.5mm}{
%         \If{$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
         
% \mybox{red}{32mm}{
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }}
%         \KwRet{ s }\;
%     }
%     }
% }

% \end{algorithm}

% \begin{algorithm}[h]
% \caption{HeightDistribution}
% \label{alg:coloredHD}
% \Class{$\mathrm{HeightDistribution(\Lambda_o)}$} {

%     \Def{$N, a[], b[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%     \uIf{$N=0$}{
%     $a[1] \gets \Lambda_k$\;
%     $b[1] \gets \Lambda_k$\;
%     $N \gets N+1$\;
%     }
%     \uElseIf{$\Lambda_k < 0$} {
%     \mybox{green}{41.5mm}{
%     \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k-b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[N+1] \gets a[N+1]-a[i] $\;
%         }
%         }
%         $b[N+1] \gets \Lambda_k$\;
%         $N \gets N+1$\;
%     }
%     }
%     \Else{
%     \mybox{yellow}{33.5mm}{
%     \mybox{red}{32mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k+b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         $b[N+1] \gets -\Lambda_k$\;}
%     }
% }
%     \Fn{$\mathrm{getP_{exit}}()$}{
%     \mybox{cyan}{28.5mm}{
%          $s \gets 0$\;
%     \mybox{red}{27mm}{
%         \For{$i \gets 1 ... N$}{
%             $s \gets s + \frac{a[i]}{\Lambda_o+b[i]}$\;
%         }
%         }
%         \KwRet{ s }\;
%         }
    
%     }
% }

% \end{algorithm}
